A comprehensive operational semantics of the SCOOP programming model

Operational semantics has established itself as a flexible but rigorous means to describe the meaning of programming languages. Oftentimes, it is felt necessary to keep a semantics small, for example to facilitate its use for model checking by avoiding state space explosion. However, omitting many details in a semantics typically makes results valid for a limited core language only, leaving a wide gap towards any real implementation. In this paper we present a full-fledged semantics of the concurrent object-oriented programming language SCOOP (Simple Concurrent Object-Oriented Programming). The semantics has been found detailed enough to guide an implementation of the SCOOP compiler and runtime system, and to detect and correct a variety of errors and ambiguities in the original informal specification and prototype implementation. In our formal specification, we use abstract data types with preconditions and axioms to describe the state, and introduce a number of special run-time operations to model the runtime system with our inference rules. This approach allows us to make our large formal specification manageable, providing a first step towards reference documents for specifying object-oriented languages based on operational semantics.

==> inference_rules_elements/call_operation_command_improved.tex <==
\inferencerule
	{Call Operation -- Command}
	{
		q \mathematicaldefinition \state.\handlerfeature(r_{0}) \\
		\overline{l} \mathematicaldefinition 
			\left\{
				\begin{split}
					& \multilinecondition{
						& q \neq p \wedge 
						\exists i \in \set{1, \ldots, n} \colon \typingenvironmentderivation{e_{i}: t \wedge \iscontrolledfeature(t)} \wedge 
						\typingenvironmentderivation{f.\formalargumentsfeature(i): (!, g, c) \wedge c.\isreferenceclasstypefeature}
					} \\
					& \indentation \tuple{\state.\requestqueuelocksfeature(p), \state.\callstacklocksfeature(p)} \\
					& \multilinecondition{
						& q \neq p \wedge
						\state.\arelockspassedfeature(q) \wedge \neg \state.\arelockspassedfeature(p) \wedge  \state.\callstacklocksfeature(p).\containsfeature(q)
					} \\
					& \indentation \tuple{\state.\requestqueuelocksfeature(p), \state.\callstacklocksfeature(p)} \\
					& \otherwisecondition \\
					& \indentation \tuple{\set{}, \set{}}
				\end{split}
			\right. \\
		\freshchanneldefinition{a}
	}
	{\configuration{p :: \calloperation(r_{0}, f, \tuple{r_{1}, \ldots, r_{n}}, \tuple{e_{1}, \ldots, e_{n}}) \statementseparator s_{p}}{\state}}
	{
		\configuration
			{
				p :: \ & \issueoperation(q, \applyoperation(a, r_{0}, f, \tuple{r_{1}, \ldots, r_{n}}, p, \overline{l})) \statementseparator \\
				& \singlelineconditionaloperation
					{\overline{l} \neq \tuple{\set{}, \set{}}}
					{\waitoperation(a)}
					{\nooperation} \statementseparator \\
				& s_{p}
			}
			{\state}
	}


==> inference_rules_elements/call_operation_query_improved.tex <==
\inferencerule
	{Call Operation -- Query}
	{
		q \mathematicaldefinition \state.\handlerfeature(r_{0}) \\
		\overline{l} \mathematicaldefinition  \tuple{\state.\requestqueuelocksfeature(p), \state.\callstacklocksfeature(p)} \\
	}
	{\configuration{p :: \calloperation(a, r_{0}, f, \tuple{r_{1}, \ldots, r_{n}}, \tuple{e_{1}, \ldots, e_{n}}) \statementseparator s_{p}}{\state}}
	{
		\configuration
			{p ::
				\issueoperation(q, \applyoperation(a, r_{0}, f, \tuple{r_{1}, \ldots, r_{n}}, p, \overline{l})) \statementseparator
				\waitoperation(a) \statementseparator
				s_{p}
			}
			{\state}
	}


==> inference_rules_elements/creation_instruction_existing_explicit_processor_improved.tex <==
\inferencerule
	{Create Instruction -- Existing Explicit Processor}
	{
		(d, h, c) \mathematicaldefinition \typefromtypingenvironment(\typingenvironment, b) \\
		h = <x> \vee h = <y.\handlerfeature> \\
		q \mathematicaldefinition 
			\left\{
				\begin{array}{ll}
					\state.\valuefeature(p, x) & \condition{t = (d, <x>, c)} \\
					\state.\handlerfeature(\state.\valuefeature(p, y)) & \condition{t = (d, <y.\handlerfeature>, c)}
				\end{array}
			\right. \\
		\state.\processorsfeature.\containsfeature(q) \\
		\begin{split}
			& \overline{g}_{required\_cs\_locks} \mathematicaldefinition \\
			& \indentation \left\{
					\begin{array}{ll}
						\set{q} & \condition{q \neq p \wedge \state.\arelockspassedfeature(q) \wedge \neg \state.\arelockspassedfeature(p) \wedge \state.\callstacklocksfeature(p).\containsfeature(q)} \\
						\set{} & \otherwisecondition
					\end{array}
				\right.
		\end{split} \\
		\forall x \in \overline{g}_{required\_cs\_locks} \colon \neg \state.\arelockspassedfeature(p) \wedge \state.\callstacklocksfeature(p).\containsfeature(x) \\
		o \mathematicaldefinition  \state.\newobjectfeature(c) \\
		\state' \mathematicaldefinition \state.\addobjectfeature(q, o) \\
		r \mathematicaldefinition  \state'.\referencefeature(o) \\
		\freshchanneldefinition{a}
	}
	{\configuration{p :: \ecreate b.f(e_{1}, \ldots, e_{n}) \statementseparator s_{p}}{\state}}
	{
		\configuration
			{
				p :: \ \multilineconditionaloperation
					{q \neq p \wedge \neg \state'.\arelockspassedfeature(q)}
					{\lockrequestqueuesoperation(\set{q})}
					{\nooperation} \statementseparator \\
				& \writevalueoperation(b.\namefeature, r) \statementseparator \\
				& b.f(e_{1}, \ldots, e_{n}) \statementseparator \\
				\multilineconditionaloperation
					{\neg f.\classtypefeature.\invariantexistsfeature \vee f.\isexportedfeature}
					{\nooperation}
					{\issueoperation(q, \evaluateoperation(a, f.\classtypefeature.\invariantfeature) \statementseparator \waitoperation(a))} \statementseparator \\
				\multilineconditionaloperation
					{q \neq p \wedge \neg \state'.\arelockspassedfeature(q)}
					{
						\begin{split}
							& \issueoperation(q, \unlockrequestqueueoperation) \statementseparator \\
							& \popobtainedrequestqueuelocksoperation 
						\end{split}
					}
					{\nooperation} \statementseparator \\
				& s_{p}
			}
			{\state'}
	}


==> inference_rules_elements/feature_application_operation_non_once_routine_or_fresh_once_routine_improved.tex <==
\inferencerule
	{Application Operation -- Non-Once Routine or Fresh Once Routine}
	{
		f \in \routinetype \wedge f.\isonceroutinefeature \rightarrow \state.\isonceroutinefreshfeature(p, f) \\
		\state.\handlerfeature(r_{0}) = p \\
		\neg \state.\passlocksfeature(q, p, \overline{l}).\arelockspassedfeature(p) \\
		\state' \mathematicaldefinition
			\left\{
				\begin{array}{ll}
					\state.\setoncefunctionnotfreshfeature(p, f, \voidvalue) & \condition{f \in \functiontype \wedge f.\isonceroutinefeature} \\
					\state.\setonceprocedurenotfreshfeature(p, f) & \condition{f \in \proceduretype \wedge f.\isonceroutinefeature} \\
					\state & \otherwisecondition
				\end{array}
			\right. \\
		\state'' \mathematicaldefinition \state'.\passlocksfeature(q, p, \overline{l}).\pushenvironmentwithfeaturefeature(p, f, r_{0}, \tuple{r_{1}, \ldots, r_{n}}) \\
		\begin{split}
			& \overline{g}_{required\_locks} \mathematicaldefinition \set{p} \cup \\
			& \indentation \setinference{x \in \processortype}{\exists i \in \set{1, \ldots, n}, g, c \colon \typingenvironmentderivation{f.\formalargumentsfeature(i): (!, g, c) \wedge c.\isreferenceclasstypefeature} \wedge x = \state''.\handlerfeature(r_{i})}
		\end{split} \\
		\begin{split}
			& \overline{g}_{required\_cs\_locks} \mathematicaldefinition \\
			& \indentation \setinference{x \in \overline{g}_{required\_locks}}{x = p \vee (x \neq p \wedge \state''.\arelockspassedfeature(x) \wedge \state''.\callstacklocksfeature(p).\containsfeature(x)}
		\end{split} \\
		\overline{g}_{required\_rq\_locks} \mathematicaldefinition \overline{g}_{required\_locks} \setminus \overline{g}_{required\_cs\_locks} \\
		\overline{g}_{missing\_rq\_ locks} \mathematicaldefinition \setinference{x \in \overline{g}_{required\_rq\_locks}}{\neg \state''.\requestqueuelocksfeature(p).\containsfeature(x)} \\
		\forall x \in \overline{g}_{required\_cs\_locks} \colon \state''.\callstacklocksfeature(p).\containsfeature(x) \\
		\freshchanneldefinition{a_{inv}} \wedge \freshchanneldefinition{a'}
	}
	{\configuration{p :: \applyoperation(a, r_{0}, f, \tuple{r_{1}, \ldots, r_{n}}, q, \overline{l}) \statementseparator s_{p}}{\state}}
	{
		\configuration
			{
				p :: \ & \checkpreconditionandlockrequestqueuesoperation(\overline{g}_{missing\_rq\_ locks}, f) \statementseparator \\
				\multilineconditionaloperation
					{f \in \functiontype \wedge f.\isonceroutinefeature}
					{
						\begin{split}
							& f.\bodyfeature \\
							& \indentation \begin{split}
								& \begin{split}
									\substitution
										{
											\resultentity \eassignment y \statementseparator
											\setonceroutinenotfreshwithresultoperation(f)
										}
										{
											\resultentity \eassignment y
										}
								\end{split} \\
								& \begin{split}
									\substitution
										{
											\ecreate \resultentity.y \statementseparator
											\setonceroutinenotfreshwithresultoperation(f)
										}
										{
											\ecreate \resultentity.y
										}
								\end{split}
							\end{split}
						\end{split}
					}
					{f.\bodyfeature} \statementseparator \\
				& \checkpostconditionandunlockrequestqueuesoperation(\overline{g}_{missing\_rq\_ locks}, f) \statementseparator \\
				\multilineconditionaloperation
					{f.\classtypefeature.\invariantexistsfeature \wedge f.\isexportedfeature}
					{\evaluateoperation(a_{inv}, f.\classtypefeature.\invariantfeature) \statementseparator \waitoperation(a_{inv})}
					{\nooperation} \statementseparator \\
				\multilineconditionaloperation
					{f \in \functiontype}
					{\readvalueoperation(\resultentityname, a') \statementseparator \returnoperation(a, a'.\datafeature, q)}
					{\returnoperation(a, q)} \statementseparator \\
				& s_{p}}
			{\state''}
	}


==> inference_rules_elements/issue_operation_separate_callback_improved.tex <==
\singlelineinferencerule
	{Issue Operation -- Separate Callback}
	{
		q \neq p \wedge \state.\arelockspassedfeature(q) \wedge \neg \state.\arelockspassedfeature(p) \wedge \state.\callstacklocksfeature(p).\containsfeature(q) \\
		\neg \state.\arelockspassedfeature(p) \\
		\state.\callstacklocksfeature(p).\containsfeature(q)		
	}
	{\configuration{p :: \issueoperation(q, s_{w}) \statementseparator s_{p} \processorseparator q :: s_{q}}{\state}}
	{\configuration{p :: s_{p} \processorseparator q :: s_{w} \statementseparator s_{q}}{\state}}


==> inference_rules_elements/issue_operation_separate_improved.tex <==
\singlelineinferencerule
	{Issue Operation -- Separate}
	{
		q \neq p \wedge \neg \state.\arelockspassedfeature(q) \\
		\neg \state.\arelockspassedfeature(p) \\
		\state.\requestqueuelocksfeature(p).\containsfeature(q)
	}
	{\configuration{p :: \issueoperation(q, s_{w}) \statementseparator s_{p} \processorseparator q :: s_{q}}{\state}}
	{\configuration{p :: s_{p} \processorseparator q :: s_{q} \statementseparator s_{w}}{\state}}

